Unmanned Aerial Vehicle Visual Detection and Tracking using Deep Neural Networks: A Performance Benchmark

Unmanned Aerial Vehicles (UAV) can pose a major risk for aviation safety, due to both negligent and malicious use. For this reason, the automated detection and tracking of UAV is a fundamental task in aerial security systems. Common technologies for UAV detection include visible-band and thermal infrared imaging, radio frequency and radar. Recent advances in deep neural networks (DNNs) for image-based object detection open the possibility to use visual information for this detection and tracking task. Furthermore, these detection architectures can be implemented as backbones for visual tracking systems, thereby enabling persistent tracking of UAV incursions. To date, no comprehensive performance benchmark exists that applies DNNs to visible-band imagery for UAV detection and tracking. To this end, three datasets with varied environmental conditions for UAV detection and tracking, comprising a total of 241 videos (331,486 images), are assessed using four detection architectures and three tracking frameworks. The best performing detector architecture obtains an mAP of 98.6% and the best performing tracking framework obtains a MOTA of 96.3%. Cross-modality evaluation is carried out between visible and infrared spectrums, achieving a maximal 82.8% mAP on visible images when training in the infrared modality. These results provide the first public multi-approach benchmark for state-of-the-art deep learning-based methods and give insight into which detection and tracking architectures are effective in the UAV domain.

==> tex/tracking.tex <==

\section{Tracking}
Tracking involves the detection of objects over subsequent video frames such that their position can be monitored and predicted. To this end, we consider the DeepSort \cite{bibid} algorithm which can be divided into four stages. In the first, we employ a multi-object detector, for which we refer the reader to \ref{label}. We utilize a motion model in the second stage, often in the form of a Kalman Filter. This enables us to impose motion constraints within our model, to capture the degrees of freedom of our objects. In our case, a UAV can be considered to have six. For a given frame $i$, the third stage associates the bounding boxes predicted (with the Kalman Filter) from frame $i-1$ to the newly detected boxes in frame $i$. As such, we are able to update our motion model to better capture the trajectory of our tracked objects. In the final stage, we employ a deep neural network to capture an appearance descriptor of a given object. This descriptor can be levied within the association stage to ensure that detected and predicted bounding boxes refer to the same object. This stage is particularly important for tracking within scenes with high occlusion (where detected bounding boxes are more likely to be incorrectly associated with predictions), and where objects leave or enter different viewpoints.

%	deepsort:
%	@inproceedings{Wojke2017simple,
%		title={Simple Online and Realtime Tracking with a Deep Association Metric},
%		author={Wojke, Nicolai and Bewley, Alex and Paulus, Dietrich},
%		booktitle={2017 IEEE International Conference on Image Processing (ICIP)},
%		year={2017},
%		pages={3645--3649},
%		organization={IEEE},
%		doi={10.1109/ICIP.2017.8296962}
%	}
